Improved Input Reprogramming for GAN Conditioning

We study the GAN conditioning problem, whose goal is to convert a pretrained unconditional GAN into a conditional GAN using labeled data. We first identify and analyze three approaches to this problem -- conditional GAN training from scratch, fine-tuning, and input reprogramming. Our analysis reveals that when the amount of labeled data is small, input reprogramming performs the best. Motivated by real-world scenarios with scarce labeled data, we focus on the input reprogramming approach and carefully analyze the existing algorithm. After identifying a few critical issues of the previous input reprogramming approach, we propose a new algorithm called InRep+. Our algorithm InRep+ addresses the existing issues with the novel uses of invertible neural networks and Positive-Unlabeled (PU) learning. Via extensive experiments, we show that InRep+ outperforms all existing methods, particularly when label information is scarce, noisy, and/or imbalanced. For instance, for the task of conditioning a CIFAR10 GAN with 1% labeled data, InRep+ achieves an average Intra-FID of 76.24, whereas the second-best method achieves 114.51.

==> cgan_failure_v0.tex <==

\paragraph{Failures of auxiliary classifier conditioning strategy}
The discriminator and generator of \ag{} learn to maximize $\lambda L_C + L_S$ and $\lambda L_C - L_S$, respectively.
Here, $L_S$ and $L_C$ model log-likelihoods of samples belonging to the real data and the correct class, and $\lambda$ is a regularization coefficient. 
In this game, $G$ might be able to maximize $\lambda L_C - L_S$ by simply learning \textit{a biased distribution} (increased $L_C$) at the cost of compromised generation quality (increased $L_S$).
Our following lemmas show that \ag{} indeed suffers from this phenomenon.
Lemma~\ref{ex:non_separable} applies for non-separable datasets (previously noted in~\citep{shu2017ac}), and Lemma~\ref{ex:separable} applies for separable datasets, which has not been \td{shown} before in the literature.
We use the Wasserstein loss for $L_S$ (W-\ag{})~\citep{martin2017wasserstein} in our examples.
\begin{lemma}[W-\ag{} may fail to learn a non-separable dataset via gradient descent]
\label{ex:non_separable}
Suppose the data follows a Gaussian mixture distribution with a known location but unknown variance. 
Furthermore, assume that a Gaussian mixture generator parameterized by its variance is trained. 
Then, the generator trained by gradient descent converges to the degenerate distribution as $\lambda \to \infty$.

\td{Suppose the data follows a Gaussian mixture distribution with a known location but unknown variance, and a Gaussian mixture generator parameterized by its variance is being trained. 
Then, the generator trained by gradient descent collapses as the weight of classification loss getting larger.
}
\end{lemma}

\begin{lemma}[\textsc{W-\ag{}} may fail to learn a separable distribution] \label{ex:separable}
Suppose real data are vertically uniform in $2$-D space: conditioned on $y \in \{\pm 1\}$, $\rvx=(\rx_1, \rx_2)=(d \cdot \ry, \ru)$ with some $d>0$ and $\ru \sim \Unif[-1,1]$. 
An auxiliary classifier is a linear classifier, passing the origin. 
We can find a single-parameter generator s.t. 1) it controls the sign of $x_1$ and range of $x_2$ according to the parameter, and 2) $L_S + \lambda L_C$ has bad critical points. 
Thus, gradient descent may not converge to the global optimum.

\td{Suppose real data are vertically uniform in $2$-D space: conditioned on $y \in \{\pm 1\}$, $\rvx=(\rx_1, \rx_2)=(d \cdot \ry, \ru)$ with some $d>0$ and $\ru \sim \Unif[-1,1]$. 
An auxiliary classifier is a linear classifier, passing the origin. 
For some single-parameter generators, gradient descent deviates from the global optimum.}
\end{lemma}

\paragraph{Failures of projection-based conditioning strategy}
The objective function of projection-based discriminator is $D(\vx, \vy; \vtheta_D) = \vy^{T}\mV\phi(\vx) + \psi(\phi(\vx))$
where $\vy$ is the one-hot encoded label vector, $\mV=[\vv_1^T;\vv_2^T;\cdots]$ is the label embedding matrix of $\rvy$, and $\phi, \psi$ are two functions to be learned. 
The objective measures the orthogonality between $\vv_y$ and $\phi(\vx)$.
Thus, even when the generator learns the correct conditional distributions, it may continue evolving to further orthogonalize the inner product term if the $\mV$ matrix is not well-chosen. 
This behavior of the generator can result in learning inexact conditional distribution, illustrated in the following lemma.
\begin{lemma}
Consider a simple projection-based CGAN with two equiprobable classes.
Assuming $\phi(\vx) = \vx$ and $\psi(\vx) = 0$, the discriminator computes $D(\vx, \vy; \vtheta_D) = \vy^{T}\mV\vx$.
We use hinge loss as in~\citep[Section 5]{miyato2018cgans}.
Then, there exist discriminator's bad embedding vectors that encourage the generator to deviate from the exact conditional distributions.%

\td{Consider a simple projection-based CGAN with two equiprobable classes.
For some simple choice of encoding functions, there exist discriminator's bad embedding vectors that encourage the generator to deviate from the exact conditional distributions}
\end{lemma}

